Enhancing Certifiable Robustness via a Deep Model Ensemble

We propose an algorithm to enhance certified robustness of a deep model ensemble by optimally weighting each base model. Unlike previous works on using ensembles to empirically improve robustness, our algorithm is based on optimizing a guaranteed robustness certificate of neural networks. Our proposed ensemble framework with certified robustness, RobBoost, formulates the optimal model selection and weighting task as an optimization problem on a lower bound of classification margin, which can be efficiently solved using coordinate descent. Experiments show that our algorithm can form a more robust ensemble than naively averaging all available models using robustly trained MNIST or CIFAR base models. Additionally, our ensemble typically has better accuracy on clean (unperturbed) data. RobBoost allows us to further improve certified robustness and clean accuracy by creating an ensemble of already certified models.

==> alg-connections.tex <==
\section{Connections to Existing Boosting Methods}
\label{sec:boost_connect}

We can formulate our proposed robustness boosting as a Forward Stage-wise Additive Modeling (FSAM) procedure~\cite{friedman2000additive} which is compatible with existing boosting framework, by designing a special ``classifier'' function and a specific loss function. Here our idea is presented in a more general framework which allows easy further extensions.

We define a new vector function $\bm{g}_t(\x) \coloneqq [\text{vec}(\bL_{t}(\x, \epsilon)) \quad \bc_t(\x, \epsilon)] \in \R^{C \times d+C}$ as the output of ``weak classifiers''. Here we explicitly show the dependency of $\x$ and $\epsilon$ for $\bL$ and $\bc$. $\epsilon$ is usually a given constant. Suppose we have $\bm{g}_t$ chosen from a set $\mathcal{G}$. The FSAM procedure then produces the boosted ``classifier'':
\begin{align*}
\bm{F}_t (\x) &= \sum\nolimits_{i=1}^t \alpha_t \bm{g}_t(\x) \\
&= \left [ \sum\nolimits_{i=1}^t \alpha_t \text{vec}(\bL_{t}(\x, \epsilon)) \quad \sum\nolimits_{i=1}^t \alpha_t \bc_t(\x, \epsilon) \right ] \\
&\coloneqq \left [ \text{vec}(\bm{\Sigma}^L) \quad \bm{\Sigma}^c \right ]
\end{align*}
where $\bm{\Sigma}^L$ and $\bm{\Sigma}^c$ are defined as the first and second part of $\bm{F}_t (\x)$ for convenience. We now design a special loss function $L(\bm{F}_t(\xk), y_k)$:
\begin{align*}
    L(\bm{F}_t(\xk), y_k) = \sum\nolimits_{j \in [C-1]} \ell (- \| \hat{\bm{\Sigma}}^L_{(j,:)} \|_q \epsilon   + \hat{\bm{\Sigma}}^c_j)
\end{align*}
where $\hat{\bm{\Sigma}}^L$ and $\hat{\bm{\Sigma}}^c$ are formed on the row difference between row $y_k$ and other rows of in same manner as in~\eqref{eq:w_diff}\eqref{eq:b_diff}. $\ell$ is some loss function that penalizes a small normalized margin, which is a surrogate of robustness. For illustration, here we sum the loss of margins of each target class $s(j,y_k), j \in [C-1]$ directly. Other entry-wise loss functions can also be incorporated into this framework easily.

In the FSAM framework, we want to choose the optimal classifier $\bm{g}_{t+1} \in \mathcal{G}$ as well as $\alpha_{t+1}$ to minimize the loss:
\begin{align*}
    (\bm{g}_{t+1}, \alpha_{t+1}) = \argmin_{\bm{g}_{t+1}, \balp_{t+1}} \sum_{k=1}^N L(\bm{F}_t(\xk) + \alpha_{t+1} \bm{g}_{t+1}, y_k)
\end{align*}

Giving an explicit solution for this minimization problem can be hard. One solvable case is the classic AdaBoost, using an exponential loss on binary classifiers. An alternative view of AdaBoost is a coordinate descent method to search for a good additive model~\cite{rosset2004boosting}, which inspires us to develop a coordinate descent based algorithm.
